Towards Continual Test-Time Adaptation of Vision-Language Models in Open-Vocabulary Semantic Segmentation

Open-vocabulary semantic segmentation (OVSS) relies on vision-language alignment to recognize arbitrary text-defined categories, yet this alignment is fragile under continual test-time distribution shift. Our diagnostic analysis reveals that entropy minimization drives patch-level class collapse, continual updates erode vision-language alignment, and redundant gradients from low-shift samples waste computation. We propose Diversify, Anchor, and Filter (DAF), a stabilization framework that augments entropy-based adaptation with a marginal diversity loss that resists collapse, a cross-modal anchor consistency loss that constrains feature drift relative to a frozen source model, and feature salience filtering that skips low-value backward passes to offset part of the source-anchor overhead. We evaluate on five datasets spanning natural scenes, autonomous driving, underwater imagery, and remote sensing with their corrupted variants. Across the evaluated continual shifts, DAF remains stable where entropy minimization collapses, improving mIoU by over 8 points on Pascal VOC20-C, over 9 points on LoveDA, and over 3 points on Foggy Cityscapes compared to the source model, and is robust to aggressive adaptation and learning rate choices.

==> sections/preliminary.tex <==
This file is intentionally left empty. The full Preliminaries content has been moved to the supplementary material (supplement.tex) and a concise summary is retained in methodology.tex.


==> tables/ctta_benchmark_fine_hori.tex <==
\begin{table*}[tb]
    \caption{Benchmark results on segmentation datasets under CTTA. Adaptation is continuous between domains, without resetting the model. Entries report mIoU (\%), averaged over seeds 0/1/2.}
    \label{tab:ctta_benchmark_fine}
    \centering
    \tiny
    \setlength\tabcolsep{3pt}
    \begin{tabular}{c|c|ccccccccccccccc|c}
        \hline
        & TIME & \multicolumn{15}{c|}{$t\xrightarrow{\;}$} & \\
        \hline
        DATASET & METHOD &
        \rotatebox[origin=c]{45}{GAUSS} & \rotatebox[origin=c]{45}{SHOT} & \rotatebox[origin=c]{45}{IMPUL} & \rotatebox[origin=c]{45}{DEFOC} & \rotatebox[origin=c]{45}{GLASS} & \rotatebox[origin=c]{45}{MOTN} & \rotatebox[origin=c]{45}{ZOOM} & \rotatebox[origin=c]{45}{SNOW} & \rotatebox[origin=c]{45}{FROST} & \rotatebox[origin=c]{45}{FOG} & \rotatebox[origin=c]{45}{BRT} & \rotatebox[origin=c]{45}{CNTRT} & \rotatebox[origin=c]{45}{ELAST} & \rotatebox[origin=c]{45}{PIXEL} & \rotatebox[origin=c]{45}{JPEG}
        & MEAN$\uparrow$\\
        \hline
        \multirow{7}{*}{\rotatebox[origin=c]{45}{VOC20-C\cite{Everingham2014ThePV}}}
        & SOURCE
        & 48.0$\pm$0.0 & 52.4$\pm$0.0 & 49.5$\pm$0.0 & 68.0$\pm$0.0 & 62.1$\pm$0.0 & 69.5$\pm$0.0 & 47.3$\pm$0.0 & 60.9$\pm$0.0 & 55.4$\pm$0.0 & 67.0$\pm$0.0 & 73.3$\pm$0.0 & 60.3$\pm$0.0 & 50.1$\pm$0.0 & 75.5$\pm$0.0 & 69.1$\pm$0.0 & 60.6 \\
        & TENT \cite{Wang2021TentFT}
        & 36.8$\pm$1.5 & 3.7$\pm$1.6 & 1.0$\pm$0.4 & 7.0$\pm$1.6 & 0.3$\pm$0.2 & 0.5$\pm$0.2 & 0.2$\pm$0.1 & 0.3$\pm$0.2 & 0.6$\pm$0.3 & 1.7$\pm$1.0 & 0.6$\pm$0.3 & 0.9$\pm$0.3 & 0.1$\pm$0.0 & 0.2$\pm$0.1 & 0.2$\pm$0.0 & 3.6 \\
        & DAF-T
        & 51.2$\pm$0.1 & 56.3$\pm$0.1 & 53.5$\pm$0.2 & 70.3$\pm$0.1 & 65.6$\pm$0.2 & 71.9$\pm$0.2 & 52.5$\pm$0.1 & 65.6$\pm$0.3 & 60.7$\pm$0.4 & 71.2$\pm$0.5 & 76.6$\pm$0.4 & 63.7$\pm$0.2 & 55.1$\pm$0.3 & 77.4$\pm$0.1 & 71.2$\pm$0.1 & 64.2 \\
        & WATT \cite{Osowiechi2024WATTWA}
        & 16.5$\pm$0.3 & 16.1$\pm$0.3 & 16.2$\pm$0.2 & 41.3$\pm$0.6 & 32.6$\pm$0.2 & 41.4$\pm$0.5 & 19.7$\pm$0.2 & 28.2$\pm$0.3 & 23.6$\pm$0.3 & 38.4$\pm$0.3 & 39.1$\pm$0.1 & 33.3$\pm$0.3 & 20.0$\pm$0.6 & 49.3$\pm$0.1 & 35.4$\pm$0.1 & 30.1 \\
        & CLIPArTT \cite{Hakim2024CLIPArTTAO}
        & 9.8$\pm$0.3 & 2.8$\pm$0.9 & 1.8$\pm$0.4 & 3.8$\pm$0.2 & 1.6$\pm$0.4 & 1.9$\pm$0.3 & 1.4$\pm$0.1 & 1.3$\pm$0.4 & 1.2$\pm$0.3 & 2.4$\pm$0.6 & 1.9$\pm$0.4 & 1.5$\pm$0.5 & 0.7$\pm$0.2 & 1.1$\pm$0.4 & 0.9$\pm$0.1 & 2.3 \\
        & MLMP \cite{Noori2025TestTimeAO}
        & 59.9$\pm$0.9 & 63.1$\pm$2.6 & 17.8$\pm$5.5 & 5.3$\pm$0.9 & 1.0$\pm$0.1 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 1.2$\pm$0.0 & 1.1$\pm$0.1 & 1.2$\pm$0.1 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 10.5 \\
        & DAF-M
        & 56.4$\pm$0.3 & 61.9$\pm$0.3 & 58.2$\pm$0.3 & 73.6$\pm$0.6 & 71.2$\pm$0.3 & 74.0$\pm$0.1 & 57.2$\pm$0.6 & 69.2$\pm$0.5 & 65.1$\pm$0.3 & 75.1$\pm$0.1 & 78.8$\pm$0.2 & 69.4$\pm$0.3 & 60.8$\pm$0.7 & 79.0$\pm$0.2 & 74.2$\pm$0.3 & 68.3 \\
        \hline
        
        \multirow{7}{*}{\rotatebox[origin=c]{45}{VOC21-C\cite{Everingham2014ThePV}}}
        & SOURCE
        & 35.7$\pm$0.0 & 38.7$\pm$0.0 & 36.8$\pm$0.0 & 44.4$\pm$0.0 & 43.4$\pm$0.0 & 46.1$\pm$0.0 & 33.4$\pm$0.0 & 42.4$\pm$0.0 & 40.9$\pm$0.0 & 45.8$\pm$0.0 & 49.8$\pm$0.0 & 42.6$\pm$0.0 & 38.7$\pm$0.0 & 49.8$\pm$0.0 & 47.5$\pm$0.0 & 42.4 \\
        & TENT \cite{Wang2021TentFT}
        & 38.9$\pm$0.3 & 43.0$\pm$0.5 & 38.5$\pm$2.3 & 40.8$\pm$2.1 & 27.7$\pm$20.2 & 23.8$\pm$19.1 & 8.3$\pm$8.2 & 4.8$\pm$1.4 & 3.9$\pm$0.2 & 4.2$\pm$0.1 & 4.5$\pm$0.4 & 4.9$\pm$0.2 & 3.5$\pm$0.0 & 3.5$\pm$0.0 & 3.5$\pm$0.0 & 16.9 \\
        & DAF-T
        & 36.4$\pm$0.1 & 39.2$\pm$0.1 & 37.2$\pm$0.1 & 43.9$\pm$0.2 & 43.3$\pm$0.0 & 45.1$\pm$0.0 & 33.8$\pm$0.1 & 42.5$\pm$0.1 & 41.4$\pm$0.2 & 46.0$\pm$0.1 & 49.2$\pm$0.2 & 42.3$\pm$0.1 & 39.0$\pm$0.1 & 48.6$\pm$0.1 & 46.0$\pm$0.1 & 42.3 \\
        & WATT \cite{Osowiechi2024WATTWA}
        & 10.5$\pm$0.3 & 10.3$\pm$0.1 & 10.1$\pm$0.1 & 29.4$\pm$0.1 & 22.1$\pm$0.2 & 29.4$\pm$0.2 & 13.5$\pm$0.1 & 18.1$\pm$0.4 & 12.9$\pm$0.4 & 23.8$\pm$0.2 & 26.1$\pm$0.3 & 22.2$\pm$0.1 & 10.9$\pm$0.2 & 34.3$\pm$0.3 & 23.3$\pm$0.1 & 19.8 \\
        & CLIPArTT \cite{Hakim2024CLIPArTTAO}
        & 7.2$\pm$0.6 & 0.9$\pm$0.3 & 0.7$\pm$0.1 & 2.4$\pm$0.3 & 0.6$\pm$0.0 & 0.9$\pm$0.2 & 0.8$\pm$0.1 & 0.8$\pm$0.1 & 0.5$\pm$0.2 & 0.7$\pm$0.2 & 0.9$\pm$0.2 & 0.8$\pm$0.2 & 0.3$\pm$0.0 & 0.3$\pm$0.1 & 0.3$\pm$0.0 & 1.2 \\
        & MLMP \cite{Noori2025TestTimeAO}
        & 40.6$\pm$0.4 & 36.0$\pm$4.2 & 3.6$\pm$0.1 & 4.5$\pm$0.3 & 3.5$\pm$0.0 & 3.5$\pm$0.0 & 3.5$\pm$0.0 & 3.5$\pm$0.0 & 3.5$\pm$0.0 & 3.7$\pm$0.1 & 3.5$\pm$0.0 & 3.8$\pm$0.1 & 3.5$\pm$0.0 & 3.5$\pm$0.0 & 3.5$\pm$0.0 & 8.3 \\
        & DAF-M
        & 38.3$\pm$0.2 & 40.9$\pm$0.1 & 39.0$\pm$0.1 & 43.8$\pm$0.2 & 44.4$\pm$0.2 & 45.2$\pm$0.1 & 35.1$\pm$0.3 & 43.4$\pm$0.3 & 42.8$\pm$0.0 & 46.8$\pm$0.1 & 49.1$\pm$0.0 & 44.1$\pm$0.2 & 40.7$\pm$0.4 & 48.2$\pm$0.1 & 45.2$\pm$0.3 & 43.1 \\
        \hline
        
        \multirow{5}{*}{\rotatebox[origin=c]{45}{BDD100K-C\cite{Yu2018BDD100KAD}}}
        & SOURCE
        & 8.7$\pm$0.0 & 10.2$\pm$0.0 & 9.7$\pm$0.0 & 21.5$\pm$0.0 & 16.3$\pm$0.0 & 22.1$\pm$0.0 & 12.9$\pm$0.0 & 19.0$\pm$0.0 & 16.1$\pm$0.0 & 28.0$\pm$0.0 & 28.3$\pm$0.0 & 18.1$\pm$0.0 & 26.1$\pm$0.0 & 24.1$\pm$0.0 & 19.5$\pm$0.0 & 18.7 \\
        & TENT \cite{Wang2021TentFT}
        & 6.5$\pm$0.2 & 0.8$\pm$0.0 & 0.7$\pm$0.0 & 1.4$\pm$0.1 & 0.7$\pm$0.0 & 0.7$\pm$0.0 & 0.7$\pm$0.0 & 0.9$\pm$0.0 & 0.9$\pm$0.0 & 1.1$\pm$0.0 & 0.7$\pm$0.0 & 0.7$\pm$0.0 & 0.7$\pm$0.0 & 0.7$\pm$0.0 & 0.7$\pm$0.0 & 1.2 \\
        & DAF-T
        & 11.9$\pm$0.0 & 14.2$\pm$0.0 & 13.2$\pm$0.0 & 21.5$\pm$0.0 & 18.4$\pm$0.0 & 21.1$\pm$0.0 & 14.8$\pm$0.0 & 18.2$\pm$0.0 & 16.1$\pm$0.0 & 25.0$\pm$0.0 & 24.4$\pm$0.0 & 17.8$\pm$0.0 & 24.1$\pm$0.0 & 21.7$\pm$0.0 & 19.0$\pm$0.0 & 18.8 \\
        & MLMP \cite{Noori2025TestTimeAO}
        & 7.1$\pm$0.1 & 1.9$\pm$0.0 & 1.8$\pm$0.0 & 2.0$\pm$0.0 & 1.8$\pm$0.0 & 1.8$\pm$0.0 & 1.8$\pm$0.0 & 1.8$\pm$0.0 & 1.9$\pm$0.0 & 1.9$\pm$0.0 & 1.8$\pm$0.0 & 1.8$\pm$0.0 & 1.8$\pm$0.0 & 1.8$\pm$0.0 & 1.8$\pm$0.0 & 2.2 \\
        & DAF-M
        & 13.2$\pm$0.1 & 15.1$\pm$0.1 & 14.0$\pm$0.0 & 21.3$\pm$0.0 & 18.2$\pm$0.1 & 21.0$\pm$0.1 & 15.2$\pm$0.0 & 18.8$\pm$0.1 & 16.3$\pm$0.0 & 26.1$\pm$0.0 & 24.9$\pm$0.0 & 19.8$\pm$0.0 & 23.5$\pm$0.0 & 21.7$\pm$0.0 & 19.2$\pm$0.0 & 19.2 \\
        \hline

        \multirow{7}{*}{\rotatebox[origin=c]{45}{COCOSTUFF10K-C\cite{Caesar2016COCOStuffTA}}}
        & SOURCE
        & 12.0$\pm$0.0 & 12.7$\pm$0.0 & 12.0$\pm$0.0 & 18.5$\pm$0.0 & 17.5$\pm$0.0 & 19.4$\pm$0.0 & 9.8$\pm$0.0 & 15.1$\pm$0.0 & 14.1$\pm$0.0 & 19.5$\pm$0.0 & 21.5$\pm$0.0 & 14.8$\pm$0.0 & 17.3$\pm$0.0 & 21.8$\pm$0.0 & 19.2$\pm$0.0 & 16.4 \\
        & TENT \cite{Wang2021TentFT}
        & 12.7$\pm$0.1 & 12.8$\pm$0.7 & 9.6$\pm$2.5 & 12.7$\pm$4.7 & 9.9$\pm$7.0 & 10.4$\pm$7.3 & 5.0$\pm$3.6 & 4.3$\pm$3.6 & 1.1$\pm$1.1 & 0.9$\pm$0.5 & 0.1$\pm$0.0 & 0.3$\pm$0.3 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 5.3 \\
        & DAF-T
        & 12.5$\pm$0.1 & 13.4$\pm$0.1 & 12.8$\pm$0.1 & 18.6$\pm$0.1 & 17.6$\pm$0.2 & 19.5$\pm$0.1 & 10.2$\pm$0.0 & 15.6$\pm$0.1 & 14.6$\pm$0.1 & 19.6$\pm$0.0 & 21.1$\pm$0.0 & 15.5$\pm$0.1 & 17.4$\pm$0.1 & 21.3$\pm$0.1 & 18.6$\pm$0.0 & 16.6 \\
        & WATT \cite{Osowiechi2024WATTWA}
        & 4.2$\pm$0.2 & 3.7$\pm$0.1 & 3.7$\pm$0.0 & 11.6$\pm$0.3 & 9.3$\pm$0.1 & 11.8$\pm$0.1 & 3.0$\pm$0.2 & 2.9$\pm$0.1 & 3.5$\pm$0.1 & 8.4$\pm$0.1 & 11.1$\pm$0.1 & 5.4$\pm$0.2 & 6.6$\pm$0.2 & 14.8$\pm$0.2 & 8.9$\pm$0.1 & 7.3 \\
        & CLIPArTT \cite{Hakim2024CLIPArTTAO}
        & 4.1$\pm$0.2 & 0.7$\pm$0.1 & 0.3$\pm$0.0 & 0.8$\pm$0.1 & 0.4$\pm$0.1 & 0.2$\pm$0.1 & 0.1$\pm$0.0 & 0.2$\pm$0.1 & 0.1$\pm$0.0 & 0.3$\pm$0.1 & 0.2$\pm$0.1 & 0.2$\pm$0.1 & 0.0$\pm$0.0 & 0.1$\pm$0.0 & 0.0$\pm$0.0 & 0.5 \\
        & MLMP \cite{Noori2025TestTimeAO}
        & 14.0$\pm$0.0 & 14.7$\pm$0.1 & 13.1$\pm$0.6 & 16.2$\pm$0.2 & 16.4$\pm$0.4 & 16.0$\pm$0.3 & 7.6$\pm$0.9 & 3.8$\pm$2.5 & 0.3$\pm$0.2 & 0.3$\pm$0.1 & 0.0$\pm$0.0 & 0.1$\pm$0.1 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 0.0$\pm$0.0 & 6.8 \\
        & DAF-M
        & 13.4$\pm$0.0 & 14.4$\pm$0.1 & 14.0$\pm$0.0 & 18.6$\pm$0.1 & 18.1$\pm$0.0 & 19.3$\pm$0.1 & 10.6$\pm$0.1 & 14.9$\pm$0.4 & 14.8$\pm$0.3 & 19.1$\pm$0.1 & 20.2$\pm$0.1 & 15.9$\pm$0.2 & 17.6$\pm$0.1 & 20.8$\pm$0.0 & 18.1$\pm$0.2 & 16.7 \\
        \hline

        \multirow{5}{*}{\rotatebox[origin=c]{45}{LoveDA-C\cite{Wang2021LoveDAAR}}}
        & SOURCE
        & 3.9$\pm$0.0 & 3.9$\pm$0.0 & 4.1$\pm$0.0 & 15.2$\pm$0.0 & 13.0$\pm$0.0 & 14.8$\pm$0.0 & 9.6$\pm$0.0 & 12.9$\pm$0.0 & 12.5$\pm$0.0 & 17.8$\pm$0.0 & 20.3$\pm$0.0 & 7.0$\pm$0.0 & 19.2$\pm$0.0 & 13.8$\pm$0.0 & 6.7$\pm$0.0 & 11.6 \\
        & TENT \cite{Wang2021TentFT}
        & 1.3$\pm$0.0 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 1.1$\pm$0.0 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 1.1$\pm$0.0 & 1.1$\pm$0.0 & 1.1$\pm$0.0 & 1.1$\pm$0.0 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 1.0$\pm$0.0 & 1.1 \\
        & DAF-T
        & 5.2$\pm$0.0 & 7.5$\pm$0.0 & 8.1$\pm$0.0 & 16.4$\pm$0.0 & 15.2$\pm$0.0 & 17.2$\pm$0.0 & 12.5$\pm$0.0 & 16.2$\pm$0.0 & 15.8$\pm$0.0 & 20.8$\pm$0.0 & 22.0$\pm$0.0 & 12.1$\pm$0.0 & 21.8$\pm$0.1 & 16.9$\pm$0.0 & 12.8$\pm$0.0 & 14.7 \\
        & MLMP \cite{Noori2025TestTimeAO}
        & 5.7$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2$\pm$0.0 & 5.2 \\
        & DAF-M
        & 6.7$\pm$0.1 & 8.3$\pm$0.0 & 10.1$\pm$0.0 & 18.4$\pm$0.0 & 17.2$\pm$0.1 & 18.7$\pm$0.1 & 14.0$\pm$0.1 & 16.2$\pm$0.0 & 15.5$\pm$0.0 & 21.9$\pm$0.1 & 24.1$\pm$0.0 & 13.2$\pm$0.1 & 23.6$\pm$0.0 & 18.4$\pm$0.1 & 14.1$\pm$0.1 & 16.0 \\
        \hline

        \multirow{7}{*}{\rotatebox[origin=c]{45}{SUIM-C\cite{islam2020semantic}}}
        & SOURCE
        & 19.0$\pm$0.0 & 22.0$\pm$0.0 & 20.1$\pm$0.0 & 29.2$\pm$0.0 & 23.1$\pm$0.0 & 24.1$\pm$0.0 & 15.7$\pm$0.0 & 21.4$\pm$0.0 & 24.0$\pm$0.0 & 30.5$\pm$0.0 & 30.1$\pm$0.0 & 24.6$\pm$0.0 & 22.1$\pm$0.0 & 29.4$\pm$0.0 & 26.3$\pm$0.0 & 24.1 \\
        & TENT \cite{Wang2021TentFT}
        & 18.9$\pm$0.0 & 21.4$\pm$0.1 & 19.3$\pm$0.1 & 30.0$\pm$0.3 & 21.7$\pm$0.2 & 26.3$\pm$0.1 & 15.7$\pm$0.2 & 20.8$\pm$0.1 & 23.0$\pm$0.1 & 29.4$\pm$0.1 & 29.2$\pm$0.5 & 16.7$\pm$4.2 & 19.6$\pm$0.4 & 20.2$\pm$5.7 & 15.1$\pm$6.6 & 21.8 \\
        & DAF-T
        & 19.4$\pm$0.1 & 22.7$\pm$0.1 & 22.0$\pm$0.2 & 29.8$\pm$0.2 & 23.5$\pm$0.5 & 24.0$\pm$1.1 & 15.7$\pm$0.1 & 22.5$\pm$0.2 & 25.3$\pm$1.0 & 30.7$\pm$0.4 & 31.6$\pm$0.2 & 26.7$\pm$0.6 & 22.9$\pm$0.1 & 30.9$\pm$0.1 & 28.4$\pm$0.2 & 25.1 \\
        & WATT \cite{Osowiechi2024WATTWA}
        & 14.8$\pm$0.5 & 16.6$\pm$0.4 & 15.1$\pm$0.4 & 18.0$\pm$0.3 & 16.1$\pm$0.6 & 19.6$\pm$0.3 & 12.6$\pm$0.2 & 14.6$\pm$0.5 & 16.4$\pm$0.4 & 21.4$\pm$0.1 & 22.4$\pm$0.1 & 12.7$\pm$0.1 & 17.3$\pm$0.3 & 23.6$\pm$1.6 & 19.8$\pm$0.3 & 17.4 \\
        & CLIPArTT \cite{Hakim2024CLIPArTTAO}
        & 18.1$\pm$0.4 & 16.5$\pm$0.9 & 12.2$\pm$0.3 & 19.8$\pm$0.2 & 16.3$\pm$1.6 & 13.5$\pm$1.9 & 10.5$\pm$0.1 & 11.0$\pm$0.6 & 11.0$\pm$0.1 & 14.0$\pm$2.2 & 12.7$\pm$1.9 & 10.3$\pm$0.0 & 10.9$\pm$0.3 & 10.6$\pm$0.1 & 10.3$\pm$0.0 & 13.2 \\
        & MLMP \cite{Noori2025TestTimeAO}
        & 14.1$\pm$0.0 & 15.7$\pm$0.0 & 14.9$\pm$0.0 & 17.6$\pm$0.1 & 14.4$\pm$0.1 & 16.2$\pm$0.3 & 10.7$\pm$0.1 & 14.5$\pm$0.3 & 12.7$\pm$0.2 & 16.5$\pm$0.4 & 16.2$\pm$0.3 & 10.4$\pm$0.1 & 12.0$\pm$0.1 & 11.2$\pm$0.3 & 10.7$\pm$0.1 & 13.9 \\
        & DAF-M
        & 14.5$\pm$0.1 & 16.8$\pm$0.1 & 15.7$\pm$0.1 & 18.5$\pm$0.9 & 15.8$\pm$0.3 & 18.5$\pm$0.2 & 11.2$\pm$0.1 & 16.2$\pm$0.3 & 18.1$\pm$0.6 & 22.2$\pm$0.2 & 24.1$\pm$0.5 & 15.3$\pm$0.2 & 17.6$\pm$0.3 & 24.4$\pm$1.0 & 19.8$\pm$0.4 & 17.9 \\
        \hline

    \end{tabular}

\end{table*}


==> tables/ctta_shuffle_pround_vitb16.tex <==
\begin{table*}[htbp]
    \caption{Domain-shuffled multi-pass CTTA on PASCAL VOC20-C \cite{Everingham2014ThePV} and LoveDA-C \cite{Wang2021LoveDAAR} using NACLIP\cite{Hajimiri2024PayAT} ViT-B/16. In each pass, we shuffled the domain order without resetting the model. Entries report mIoU (\%). "-" indicates OOM.}
    \label{tab:ctta_shuffle_pround_vitb16}
    \begin{center}
    \footnotesize
    \setlength\tabcolsep{4pt}
    \begin{tabular}{l|cc|c|cc|c}
        \toprule
        \multirow{2}{*}{METHOD} & \multicolumn{3}{c|}{\textbf{VOC20-C}} & \multicolumn{3}{c}{\textbf{LoveDA-C}} \\
        \cline{2-7}
         & Pass 1 & Pass 2 & Mean$\uparrow$ & Pass 1 & Pass 2 & Mean$\uparrow$ \\
        \midrule
        SOURCE      & 60.6 & 60.6 & 60.6 & 11.6 & 11.6 & 11.6 \\
        TENT        & 4.8 & 0.3 & 2.6 & 1.1 & 1.0 & 1.1 \\
        WATT        & 29.9 & 30.2 & 30.1 & - & - & - \\
        CLIPArTT    & 2.0 & 0.8 & 1.4 & - & - & - \\
        MLMP        & 22.7 & 1.1 & 11.9 & 5.2 & 5.2 & 5.2 \\
        \midrule
        \rowcolor{gray!15}DAF-T     & 64.1 & 62.4 & 63.3 & 14.9 & 15.5 & 15.2 \\
        \rowcolor{gray!15}DAF-M     & 68.3 & 65.8 & 67.1 & 16.3 & 16.9 & 16.6 \\
        \bottomrule
    \end{tabular}
    \end{center}
\end{table*}


==> tables/driving_shuffle_pround.tex <==
\begin{table*}[htbp]
    \caption{Dataset-shuffled multi-pass CTTA on Cityscapes-C \cite{Cordts2016TheCD}, ACDC\cite{Sakaridis2021ACDCTA}, and Dark Zurich \cite{Sakaridis2019GuidedCM} with NACLIP\cite{Hajimiri2024PayAT} ViT-B/32. In each pass, we shuffled the order of three datasets without resetting the model. Entries report mIoU (\%).}
    \label{tab:driving_shuffle_pround}
    \begin{center}
    \footnotesize
    \setlength\tabcolsep{3pt}
    \begin{tabular}{l|cccccccccc|c}
        \toprule
        \multirow{2}{*}{METHOD} & \multicolumn{11}{c}{Cityscapes\cite{Cordts2016TheCD}/ACDC\cite{Sakaridis2021ACDCTA}/Dark Zurich \cite{Sakaridis2019GuidedCM}} \\
        \cline{2-12}
         & Pass 1 & Pass 2 & Pass 3 & Pass 4 & Pass 5 & Pass 6 & Pass 7 & Pass 8 & Pass 9 & Pass 10 & Mean$\uparrow$ \\
        \midrule
        SOURCE      & 23.0 & 23.0 & 23.0 & 23.0 & 23.0 & 23.0 & 23.0 & 23.0 & 23.0 & 23.0 & 23.0 \\
        TENT        & 23.5 & 23.4 & 23.4 & 23.7 & 23.6 & 23.3 & 23.1 & 22.8 & 22.5 & 21.9 & 23.0 \\
        MLMP        & 25.0 & 23.4 & 22.9 & 22.6 & 23.2 & 22.5 & 22.5 & 21.8 & 21.0 & 21.0 & 22.6 \\
        \midrule
        \rowcolor{gray!15}DAF-T & 23.3 & 23.6 & 23.6 & 23.4 & 23.4 & 23.1 & 23.2 & 23.2 & 22.8 & 23.0 & 23.2 \\
        \rowcolor{gray!15}DAF-M & 25.7 & 25.6 & 25.1 & 24.4 & 23.9 & 23.6 & 23.6 & 23.4 & 23.1 & 23.0 & 24.1 \\
        \bottomrule
    \end{tabular}
    \end{center}
\end{table*}


==> tables/loveda_domain_gen.tex <==
\begin{table*}[htbp]
    \caption{Domain generalization (forward transfer). We perform CTTA on LoveDA-C\cite{Wang2021LoveDAAR} domains except for the last 5 domains. We directly evaluate on them using the adapted weights. Entries report mIoU (\%).}
    \label{tab:loveda_domain_gen}
    \begin{center}
    \footnotesize
    \setlength\tabcolsep{6pt}
    \begin{tabular}{l|ccccc|c}
        \hline
         METHOD
         & \rotatebox[origin=c]{45}{BRT} & \rotatebox[origin=c]{45}{CNTRT} & \rotatebox[origin=c]{45}{ELAST} & \rotatebox[origin=c]{45}{PIXEL} & \rotatebox[origin=c]{45}{JPEG} & Mean$\uparrow$ \\
        \hline
        SOURCE      & 20.3 & 7.0 & 19.2 & 13.8 & 6.7 & 13.4 \\
        TENT        & 1.2 & 1.0 & 1.0 & 1.0 & 1.0 & 1.1 \\
        + AF      & 23.0 & 10.8 & 23.0 & 15.8 & 10.7 & 16.7 \\
        WATT        & - & - & - & - & - & - \\
        CLIPArTT    & - & - & - & - & - & - \\
        MLMP        & 5.2 & 5.2 & 5.2 & 5.2 & 5.2 & 5.2 \\
        + AF      & 25.3 & 11.9 & 24.7 & 18.5 & 12.9 & 18.7 \\
        \hline
    \end{tabular}
    \end{center}
\end{table*}

==> tables/loveda_efficiency.tex <==
\begin{table*}[htbp]
    \caption{Adaptation efficiency of CTTA methods on LoveDA-C\cite{Wang2021LoveDAAR} using CLIP ViT-B/16. Each image is divided into $224{\times}224$ block patches as input to the CLIP model, with 64 patches per image. Each domain has $S{=}107008$ patches with batch size 8, evaluated on an AMD Instinct MI200 GPU. FORWARD and BACKWARD denote the total number of forward and backward passes per domain, expressed in terms of $S$. TIME is the per-domain adaptation time in seconds.}
    \label{tab:loveda_efficiency}
    \begin{center}
    \footnotesize
    \setlength\tabcolsep{6pt}
    \begin{tabular}{l|cccc}
        \hline
         METHOD & FORWARD & BACKWARD & TIME (s) & mIoU \\
        \hline
        SOURCE      & $1.0S$ & $0$       & 532.3 & 11.6 \\
        TENT        & $1.0S$ & $1.0S$    & 656.0 & 1.1 \\
        + AF      & $2.0S$ & $0.7S$    & 725.9 & 14.7 \\
        WATT        & -      & -         & -     & - \\
        CLIPArTT    & -      & -         & -     & - \\
        MLMP        & $1.0S$ & $1.0S$    & 763.0 & 5.2 \\
        + AF      & $2.0S$ & $0.7S$    & 815.0 & 16.0 \\
        \hline
    \end{tabular}
    \end{center}
\end{table*}

==> tables/loveda_longterm_pround.tex <==
\begin{table*}[htbp]
    \caption{Domain-shuffled multi-pass CTTA on LoveDA-C\cite{Wang2021LoveDAAR}. In each pass, we randomize the domain order without resetting the model. Entries report mIoU (\%).}
    \label{tab:loveda_longterm_pround}
    \begin{center}
    \footnotesize
    \setlength\tabcolsep{6pt}
    \begin{tabular}{l|ccc|c}
        \hline
        \multirow{1}{*}{METHOD}
         & Pass 1 & Pass 2 & Pass 3 & Mean$\uparrow$ \\
        \hline
        SOURCE      & 11.6 & 11.6 & 11.6 & 11.6 \\
        TENT        & 1.1 & 1.0 & 1.0 & 1.0 \\
        + AF      & 14.9 & 15.5 & 15.7 & 15.4 \\
        WATT        & - & - & - & - \\
        CLIPArTT    & - & - & - & - \\
        MLMP        & 5.2 & 5.2 & 5.2 & 5.2 \\
        + AF      & 16.3 & 16.9 & 17.0 & 16.7 \\
        \hline
    \end{tabular}
    \end{center}
\end{table*}

==> tables/voc20_domain_gen.tex <==
\begin{table*}[htbp]
    \caption{Domain generalization (forward transfer). We perform CTTA on PASCAL VOC20-C \cite{Everingham2014ThePV} domains except for the last 5 domains. We directly evaluate on them using the adapted weights. Entries report mIoU (\%).}
    \label{tab:voc_domain_gen}
    \begin{center}
    \footnotesize
    \setlength\tabcolsep{6pt}
    \begin{tabular}{l|ccccc|c}
        \hline
         METHOD
         & \rotatebox[origin=c]{45}{BRT} & \rotatebox[origin=c]{45}{CNTRT} & \rotatebox[origin=c]{45}{ELAST} & \rotatebox[origin=c]{45}{PIXEL} & \rotatebox[origin=c]{45}{JPEG} & Mean$\uparrow$ \\
        \hline
        SOURCE      & 73.3 & 60.3 & 50.1 & 75.5 & 69.1 & 65.6 \\
        TENT        & 0.3 & 1.3 & 0.1 & 0.2 & 0.2 & 0.4 \\
        + AF      & 76.9 & 62.5 & 55.2 & 78.0 & 71.6 & 68.9 \\
        WATT        & 75.1 & 59.5 & 47.1 & 76.1 & 69.6 & 65.5 \\
        CLIPArTT    & 1.6 & 1.8 & 0.7 & 1.0 & 1.0 & 1.2 \\
        MLMP        & 1.2 & 1.6 & 1.0 & 1.0 & 1.0 & 1.2 \\
        + AF      & 78.4 & 66.6 & 56.9 & 78.3 & 72.4 & 70.5 \\
        \hline
    \end{tabular}
    \end{center}
\end{table*}

==> tables/voc20_efficiency_vitb16.tex <==
\begin{table*}[htbp]
    \caption{Adaptation efficiency of CTTA methods on PASCAL VOC20-C \cite{Everingham2014ThePV} using NACLIP\cite{Hajimiri2024PayAT} ViT-B/16. Each image is divided into $224{\times}224$ block patches as input to the CLIP model. Each domain has $S{=}1456$ patches with batch size 8, evaluated on an AMD Instinct MI200 GPU. Forward and Backward denote the total number of forward and backward passes per domain, expressed in terms of $S$. Time (s) is the per-domain adaptation time in seconds.}
    \label{tab:voc20_efficiency}
    \begin{center}
    \footnotesize
    \setlength\tabcolsep{6pt}
    \begin{tabular}{l|ccc|c}
        \toprule
         Method & Forward & Backward & Time (s) & mIoU \\
        \midrule
        SOURCE      & $1.0S$ & $0$       & 61.7  & 60.6 \\
        TENT        & $1.0S$ & $1.0S$    & 58.8  & 3.6 \\
        WATT        & $50.0S$ & $25.0S$  & 674.0 & 30.1 \\
        CLIPArTT    & $2.0S$ & $1.0S$    & 306.5 & 2.3 \\
        MLMP        & $1.0S$ & $1.0S$    & 59.7  & 10.5 \\
        \midrule
        \rowcolor{gray!15}DAF-T      & $2.0S$ & $0.7S$    & 65.1  & 64.2 \\
        \rowcolor{gray!15}DAF-M      & $2.0S$ & $0.7S$    & 57.3  & 68.3 \\
        \bottomrule
    \end{tabular}
    \end{center}
\end{table*}

==> tables/voc20_longterm_pround.tex <==
\begin{table*}[htbp]
    \caption{Domain-shuffled multi-pass CTTA on PASCAL VOC20-C \cite{Everingham2014ThePV}. In each pass, we randomize the domain order without resetting the model. Entries report mIoU (\%).}
    \label{tab:voc_longterm_pround}
    \begin{center}
    \footnotesize
    \setlength\tabcolsep{6pt}
    \begin{tabular}{l|ccc|c}
        \hline
        \multirow{1}{*}{METHOD}
         & Pass 1 & Pass 2 & Pass 3 & Mean$\uparrow$ \\
        \hline
        SOURCE      & 60.6 & 60.6 & 60.6 & 60.6 \\
        TENT        & 4.8 & 0.3 & 0.2 & 1.8 \\
        + AF      & 64.1 & 62.4 & 61.1 & 62.5 \\
        WATT        & 29.9 & 30.2 & 30.1 & 30.1 \\
        CLIPArTT    & 2.0 & 0.8 & 0.7 & 1.2 \\
        MLMP        & 22.7 & 1.1 & 1.0 & 8.3 \\
        + AF      & 68.3 & 65.8 & 63.2 & 65.8 \\
        \hline
    \end{tabular}
    \end{center}
\end{table*}
